Towards the Safe Programming of Wireless Sensor Networks

Sensor networks are rather challenging to deploy, program, and debug. Current programming languages for these platforms suffer from a significant semantic gap between their specifications and underlying implementations. This fact precludes the development of (type-)safe applications, which would potentially simplify the task of programming and debugging deployed networks. In this paper we define a core calculus for programming sensor networks and propose to use it as an assembly language for developing type-safe, high-level programming languages.

==> eptcsdata.tex <==
\providecommand{\event}{Alastair R. Beresford and Simon Gay (Eds.): Programming Language\\ Approaches to Concurrency and Communication-cEntric Software}
\providecommand{\volume}{17}
\providecommand{\anno}{2010}
\providecommand{\firstpage}{49}
\providecommand{\eid}{5}

